Multi-class Classification without Multi-class Labels

This work presents a new strategy for multi-class classification that requires no class-specific labels, but instead leverages pairwise similarity between examples, which is a weaker form of annotation. The proposed method, meta classification learning, optimizes a binary classifier for pairwise similarity prediction and through this process learns a multi-class classifier as a submodule. We formulate this approach, present a probabilistic graphical model for it, and derive a surprisingly simple loss function that can be used to learn neural network-based models. We then demonstrate that this same framework generalizes to the supervised, unsupervised cross-task, and semi-supervised settings. Our method is evaluated against state of the art in all three learning paradigms and shows a superior or comparable accuracy, providing evidence that learning multi-class classification without multi-class labels is a viable learning option.

==> elaboration.tex <==
\section{Elaboration}

==> pgm.tex <==

\section{A probabilistic graphical model interpretation} \label{graphical_model_explain}
\yhnote {Move the equations to appendix if too long?} \zlnote{Storywise, it is quite weird to go through the same thing again in a different formulation. What equation 5 ends up with basically is the same as equation 3. I would suggest to merge these two sections together into one. For example, starting from this section and then with one paragraph simplifying it into equation 3.}\zknote{I agree}\yhnote{I think Section 2 is self-explained. Merging 2.1 to 2 only mess up section 2. I will just move 2.1 into appendix.}

\begin{figure}
  \centering
  \includegraphics[clip, trim=3.5cm 3.2cm 3.5cm 3.2cm, width=.4\textwidth]{fig/graphical_model.pdf} 
  \caption{Graphical representation for the meta classification task; $X_i$ represents the node of input data, $Y_i$ represents the class label, $S_{ij}$ is a pairwise information between instances $i$ and $j$, and $\theta$ represents the neural network parameters.}\label{fig:graphical_model}
\end{figure}

In figure \ref{fig:graphical_model}, we use $\vec{X}=\{X_1,..,X_n\}$, $\vec{Y}=\{Y_1,..,Y_n\}$, and $\vec{S} = \{S_{ij}\}_{1 \leq i,j \leq n}$ to represent the nodes for samples, class labels, and pairwise similarities, respectively. In the model, we have $Y_i \in \{1,2,..,C\}$ and $S_{ij} \in \{0,1\}$. Then we have $\pr{S_{ij}=1|Y_i,Y_j} = 1$ when $Y_i = Y_j$ and zero probability otherwise. Similarly, when $Y_i \neq Y_j$, $\pr{S_{ij}=0|Y_i,Y_j} = 1$. The output of a discriminative classifier with parameters $\theta$ is $f(x_i;\theta) = \pr{Y_i | X_i; \theta}$. Now we describe the likelihood of how the model explains the observed labeling (either with class labeling or pairwise labeling).

\begin{align} \label{eq:ccl_likelihood}
\llh (\theta ; \vec{X}, \vec{Y}, \vec{S}) &= \pr{\vec{X}, \vec{Y}, \vec{S} ; \theta} = \pr{\vec{S} | \vec{Y}} \pr{\vec{Y} | \vec{X} ; \theta} \pr{\vec{X}} 
\end{align}

It is easy to see that when $\vec{Y}$ is observed, the likelihood can be calculated by marginalizing over $\vec{S}$, which can lead to multi-class cross entropy when taking a negative logarithm of the likelihood.

Now we consider a special case of the meta classification learning scenario where $\vec{S}$ is fully observed while $\vec{Y}$ is unknown. Calculating the likelihood needs to marginalize $\vec{Y}$ by computing $\sum_{\vec{Y}}\pr{\vec{S} | \vec{Y}} \pr{\vec{Y} | \vec{X} ; \theta}$ , which is intractable. The pairwise term $\pr{\vec{S} | \vec{Y}}=\prod_{i,j}\pr{S_{ij} | Y_i,Y_j}$ makes all $Y_i$ dependent on each other and prohibits efficient factorization. Thus, we approximate the computation by imposing additional independences such that $\sij{i}{j} \perp \vec{S} \setminus \{ \sij{i}{j}\} | \x{i},\x{j}$. Now we can compute the likelihood with the observed nodes $X_i=x_i$ and $S_{ij}=s_{ij}$:

\begin{align}
\llh (\theta ; \vec{X}, \vec{S}) &\approx \sum_{\vec{Y}}\pr{\vec{S} | \vec{Y}} \pr{\vec{Y} | \vec{X} ; \theta} \\
%&\approx \prod_{i,j}  \sum_{Y_i, Y_j} \pr{Y_i | x_i; \theta} \pr{Y_j | x_j;\theta} \pr{s_{ij} | Y_i, Y_j} \\
&\approx \prod_{i,j} \Big( \sum_{Y_i=Y_j} \pr{Y_i|x_i;\theta} \pr{Y_j|x_j;\theta} \mathbbm{1}[s_{ij}=1] + \sum_{Y_i \neq Y_j} \pr{Y_i|x_i;\theta} \pr{Y_j|x_j;\theta} \mathbbm{1}[s_{ij}=0] \Big). \label{eq:ccl_likelihood_b}
\end{align}

It is straightforward to take a negative logarithm on equation \ref{eq:ccl_likelihood_b} and derive a loss function equal to the equation \ref{eq:meta_criterion}, except that equation \ref{eq:ccl_likelihood_b} has a binarized $s_{ij}$. Equation \ref{eq:ccl_likelihood_b} provides a view from the perspective of probabilistic graphical models and a likelihood explanation for the interchangeability between using class labeling and pairwise labeling for learning classifiers. It also allows us to relate our formulation to constrained clustering \citep{Basu2008}, which uses pairwise constraints (must-link and cannot link) in the optimization of a clustering criterion. In fact, equation \ref{eq:ccl_likelihood_b} can also apply to a constrained clustering, since the number of output nodes $K$ in our neural network is not required to be equal to the number of classes $C$, as this quantity is unknown in unsupervised learning. This clustering perspective naturally extends the application from a supervised learning to an unsupervised or semi-supervised learning setting.

